Learning a Decision Tree Algorithm with Transformers

Decision trees are renowned for their ability to achieve high predictive performance while remaining interpretable, especially on tabular data. Traditionally, they are constructed through recursive algorithms, where they partition the data at every node in a tree. However, identifying a good partition is challenging, as decision trees optimized for local segments may not yield global generalization. To address this, we introduce MetaTree, a transformer-based model trained via meta-learning to directly produce strong decision trees. Specifically, we fit both greedy decision trees and globally optimized decision trees on a large number of datasets, and train MetaTree to produce only the trees that achieve strong generalization performance. This training enables MetaTree to emulate these algorithms and intelligently adapt its strategy according to the context, thereby achieving superior generalization performance.

==> preamble.tex <==
\usepackage{graphicx}
\usepackage{float}

% colors
\usepackage[dvipsnames]{xcolor}
\usepackage[citecolor=CadetBlue, linkcolor=CadetBlue,colorlinks=true, urlcolor=CadetBlue]{hyperref}
% \definecolor{mygray}{gray}{0.5}
% \definecolor{cblue}{RGB}{8, 85, 153}
% \definecolor{darkblue}{RGB}{1, 43, 112}
% \definecolor{darkorange}{RGB}{197,90,17}
% \newcommand{\cblue}[1]{{\textcolor{cblue}{#1}}}
% \definecolor{cgreen}{RGB}{8, 153, 83}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{booktabs}
\usepackage{longtable}
\usepackage{placeins} %FloatBarrier
\usepackage{makecell}
\usepackage{multirow}

% \usepackage[hyperpageref]{backref}
% % \renewcommand*{\backref}[1]{\ifx#1\relax \else Page #1 \fi}
% \renewcommand*{\backrefalt}[4]{%
%     \ifcase #1 \footnotesize{(Not cited.)}%
%     \or        \footnotesize{(Cited on page~#2.)}%
%     \else      \footnotesize{(Cited on pages~#2.)}%
%     \fi}


\newcommand{\cs}[1]{{\textcolor{cblue}{#1}}}
% \usepackage{changepage}


\usepackage[capitalize]{cleveref}
\usepackage{array}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\usepackage{cleveref}

\usepackage{fontawesome}

\newcommand{\bfp}[1]{(\textbf{#1})}

\usepackage{adjustbox}

\usepackage{tabularx}

\newcommand{\blank}{\underline{\hspace{15pt}}}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\crefname{definition}{Definition}{Definitions}%
\crefname{section}{Sec.}{Secs.}%
% \let\olddefinition\mydefinition
% \renewcommand{\definition}{%
  %\crefalias{theorem}{nlem}% Theorem counter now looks like lemma
%   \olddefinition}
% \theorembodyfont{}

\usepackage{scrextend} % for addmargin
\usepackage{cite}
% \usepackage[noadjust]{cite}


% \renewcommand{\boxed}[1]{\text{\fboxsep=.2em\fbox{\m@th$\displaystyle#1$}}}

\newcommand{\err}[1]{\tiny $\pm${#1}}
\usepackage{makecell}

\newcommand{\node}{\mathfrak{t}}
\renewcommand{\dim}{d}
\newcommand{\nsamples}{n}
\newcommand{\coordindices}{[\dim]}
\newcommand{\sampindices}{[\nsamples]}
\newcommand{\hypercube}[1][d]{\braces{0,1}^{#1}}
\newcommand{\uniform}{\mu}
\newcommand{\measure}{\nu}
\newcommand{\risk}{\mathcal{R}}
\newcommand{\oraclerisk}{\mathcal{R}^*}
\newcommand{\vol}{\textnormal{Vol}}
\newcommand{\hamball}{B_{H}}
\newcommand{\funcclass}{\mathcal{F}}
\newcommand{\indep}{\perp \!\!\! \perp}

\newcommand{\bh}{\mathbf{h}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\boldy}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\beps}{\boldsymbol{\epsilon}}
\newcommand{\beeta}{\boldsymbol{\eta}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}

% Common symbols
% \newcommand{\R}{\mathbb{R}}
% \renewcommand{\P}{\mathbb{P}}
% \newcommand{\E}{\mathbb{E}}
% \newcommand{\indicator}{\mathbf{1}}
% \newcommand{\Var}{\textnormal{Var}}
% \newcommand{\Cov}{\textnormal{Cov}}
% \newcommand{\KL}{\textnormal{KL}}
% \newcommand{\diag}{\textnormal{diag}}
% \newcommand{\trace}{\textnormal{Tr}}
% \newcommand{\grad}{\nabla}
% \DeclareMathOperator*{\argmin}{\arg\!\min}

% \usepackage{fontawesom5}
\usepackage{changepage}   % for the adjustwidth environment
\newenvironment{smallindent}{\begin{adjustwidth}{0.3cm}{}}{\end{adjustwidth}}



==> tex/figures/train_methodology_figure.tex <==
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=0.8\linewidth, keepaspectratio]{img/autotree_fig3.pdf}
    \end{center}
    \caption{\method's training involves a two-phase learning curriculum: in the first phase, the focus is exclusively on learning from the optimized GOSDT trees, to closely emulate the behavior of GOSDT algorithm. 
    Then in the second phase, the training process incorporates data from both the GOSDT and CART trees, generating the ones that have better generalization capabilities. }
    %The generation of a decision tree involves in recursively calling \method{}, as shown in (a), but \mathod{} can only observe the current state of the dataset and make its decision preemptively. }
    \label{fig:autotree_methodology}
\end{figure}

==> tex/figures/xor_example.tex <==
\begin{figure}
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{img/gpt_lens.pdf}
        \caption{Logit-lens probing of \method on an XOR Level 1 problem. \yufan{REMEMBER to update the paragraphs}}
        \label{fig:gpt_lens}
    \end{subfigure}\hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, keepaspectratio]{img/layer_corr.pdf}
        \caption{The output correlation analysis between the final split and each layer's splits of \method across 91 left-out datasets. }
        \label{fig:per_layer_gptlens}
    \end{subfigure}
    \caption{Exploratory analysis of \method}
    \label{fig:xor_example}
\end{figure}

==> tex/tables/train_dataset_information.tex <==
\topcaption{List of 541 datasets used in \method's training.}\small

\begin{supertabular}{p{0.35\linewidth}|p{0.15\linewidth}|p{0.1\linewidth}|p{0.15\linewidth}}
\hline
\textbf{Dataset} & \textbf{Entries} & \textbf{Dim.} & \textbf{Classes} \\
\hline
BNG spectf test  & 1000000 & 44 & 2 \\
BNG adult  & 1000000 & 2 & 2 \\
BNG eucalyptus  & 1000000 & 14 & 5 \\
BNG Australian  & 1000000 & 14 & 2 \\
BNG SPECTF  & 1000000 & 44 & 2 \\
Agrawal1 & 1000000 & 6 & 2 \\
BNG anneal 1000 5  & 1000000 & 6 & 6 \\
BNG anneal 1000 10  & 1000000 & 6 & 6 \\
BNG anneal 5000 1  & 1000000 & 6 & 6 \\
BNG anneal 1000 1  & 1000000 & 6 & 6 \\
codrnaNorm & 488565 & 8 & 2 \\
BNG anneal 5000 5  & 1000000 & 6 & 6 \\
BNG anneal 5000 10  & 1000000 & 6 & 6 \\
BNG anneal 10000 1  & 1000000 & 6 & 6 \\
BNG anneal 10000 5  & 1000000 & 6 & 6 \\
BNG anneal 10000 10  & 1000000 & 6 & 6 \\
BNG anneal ORIG 1000 1  & 1000000 & 6 & 6 \\
BNG anneal ORIG 1000 5  & 1000000 & 6 & 6 \\
BNG anneal ORIG 1000 10  & 1000000 & 6 & 6 \\
BNG anneal ORIG 5000 1  & 1000000 & 6 & 6 \\
BNG anneal ORIG 5000 5  & 1000000 & 6 & 6 \\
BNG anneal ORIG 5000 10  & 1000000 & 6 & 6 \\
BNG anneal ORIG 10000 1  & 1000000 & 6 & 6 \\
BNG anneal ORIG 10000 5  & 1000000 & 6 & 6 \\
BNG anneal ORIG 10000 10  & 1000000 & 6 & 6 \\
BNG autos 1000 1  & 1000000 & 15 & 7 \\
BNG autos 1000 5  & 1000000 & 15 & 7 \\
BNG autos 1000 10  & 1000000 & 15 & 7 \\
BNG autos 5000 1  & 1000000 & 15 & 7 \\
BNG autos 5000 5  & 1000000 & 15 & 7 \\
BNG autos 5000 10  & 1000000 & 15 & 7 \\
BNG autos 10000 1  & 1000000 & 15 & 7 \\
BNG autos 10000 5  & 1000000 & 15 & 7 \\
BNG autos 10000 10  & 1000000 & 15 & 7 \\
BNG lymph 1000 1  & 1000000 & 3 & 4 \\
BNG lymph 1000 5  & 1000000 & 3 & 4 \\
BNG lymph 1000 10  & 1000000 & 3 & 4 \\
BNG lymph 5000 1  & 1000000 & 3 & 4 \\
BNG lymph 5000 5  & 1000000 & 3 & 4 \\
BNG lymph 5000 10  & 1000000 & 3 & 4 \\
BNG lymph 10000 1  & 1000000 & 3 & 4 \\
BNG lymph 10000 5  & 1000000 & 3 & 4 \\
BNG lymph 10000 10  & 1000000 & 3 & 4 \\
PizzaCutter3 & 1043 & 37 & 2 \\
PieChart3 & 1077 & 37 & 2 \\
artificial characters & 10218 & 7 & 10 \\
banana & 5300 & 2 & 2 \\
bank marketing & 45211 & 7 & 2 \\
banknote authentication & 1372 & 4 & 2 \\
cardiotocography & 2126 & 35 & 10 \\
eeg eye state & 14980 & 14 & 2 \\
first order theorem proving & 6118 & 51 & 6 \\
gas drift & 13910 & 128 & 6 \\
gas drift different concentrations & 13910 & 129 & 6 \\
hill valley & 1212 & 100 & 2 \\
nomao & 34465 & 89 & 2 \\
ozone level 8hr & 2534 & 72 & 2 \\
phoneme & 5404 & 5 & 2 \\
qsar biodeg & 1055 & 41 & 2 \\
ringnorm & 7400 & 20 & 2 \\
wall robot navigation & 5456 & 24 & 4 \\
spoken arabic digit & 263256 & 14 & 10 \\
skin segmentation & 245057 & 3 & 2 \\
steel plates fault & 1941 & 33 & 2 \\
twonorm & 7400 & 20 & 2 \\
volcanoes a1 & 3252 & 3 & 5 \\
volcanoes a2 & 1623 & 3 & 5 \\
volcanoes a3 & 1521 & 3 & 5 \\
volcanoes a4 & 1515 & 3 & 5 \\
volcanoes d1 & 8753 & 3 & 5 \\
volcanoes d2 & 9172 & 3 & 5 \\
volcanoes d3 & 9285 & 3 & 5 \\
volcanoes d4 & 8654 & 3 & 5 \\
volcanoes e2 & 1080 & 3 & 5 \\
volcanoes e1 & 1183 & 3 & 5 \\
volcanoes e3 & 1277 & 3 & 5 \\
volcanoes e5 & 1112 & 3 & 5 \\
autoUniv au4 2500 & 2500 & 58 & 3 \\
volcanoes e4 & 1252 & 3 & 5 \\
autoUniv au7 1100 & 1100 & 8 & 5 \\
autoUniv au6 1000 & 1000 & 37 & 8 \\
Diabetes130US & 101766 & 13 & 3 \\
numerai28 6 & 96320 & 21 & 2 \\
thyroid allhyper & 2800 & 6 & 5 \\
thyroid allhypo & 2800 & 6 & 5 \\
thyroid allrep & 2800 & 6 & 5 \\
thyroid allbp & 2800 & 6 & 5 \\
thyroid dis & 2800 & 6 & 5 \\
thyroid ann & 3772 & 21 & 3 \\
clean2 & 6598 & 168 & 2 \\
fars & 100968 & 14 & 8 \\
wine quality white & 4898 & 11 & 7 \\
shuttle & 58000 & 9 & 7 \\
wine quality red & 1599 & 11 & 6 \\
churn & 5000 & 16 & 2 \\
allbp & 3772 & 6 & 3 \\
Run or walk information & 88588 & 6 & 2 \\
wilt & 4839 & 5 & 2 \\
jungle chess 2pcs endgame lion elephant & 4704 & 20 & 3 \\
jungle chess 2pcs endgame rat rat & 3660 & 20 & 2 \\
jungle chess 2pcs endgame lion lion & 2352 & 20 & 2 \\
sylvine & 5124 & 20 & 2 \\
jungle chess 2pcs raw endgame complete & 44819 & 6 & 3 \\
MiniBooNE & 130064 & 50 & 2 \\
ada & 4147 & 48 & 2 \\
jannis & 83733 & 54 & 4 \\
volkert & 58310 & 180 & 10 \\
FOREX eurchf minute Close & 375840 & 10 & 2 \\
FOREX audchf hour High & 43825 & 10 & 2 \\
microaggregation2 & 20000 & 20 & 5 \\
FOREX eurhkd minute High & 375840 & 10 & 2 \\
FOREX eurusd minute Close & 375840 & 10 & 2 \\
FOREX eurcad hour High & 43825 & 10 & 2 \\
FOREX eurnzd day High & 1832 & 10 & 2 \\
FOREX eurpln minute High & 375840 & 10 & 2 \\
FOREX eurhuf hour High & 43825 & 10 & 2 \\
FOREX eurcad day Close & 1834 & 10 & 2 \\
FOREX usdjpy minute High & 375840 & 10 & 2 \\
FOREX audjpy hour High & 43825 & 10 & 2 \\
FOREX eurjpy day High & 1832 & 10 & 2 \\
FOREX eurusd day High & 1837 & 10 & 2 \\
FOREX audcad day High & 1834 & 10 & 2 \\
FOREX chfjpy day Close & 1832 & 10 & 2 \\
FOREX eurcad day High & 1834 & 10 & 2 \\
FOREX usdjpy day Close & 1835 & 10 & 2 \\
FOREX cadchf hour High & 43825 & 10 & 2 \\
FOREX audusd day High & 1834 & 10 & 2 \\
FOREX usdcad hour Close & 43825 & 10 & 2 \\
FOREX cadjpy minute High & 375840 & 10 & 2 \\
FOREX usdchf day High & 1835 & 10 & 2 \\
FOREX chfjpy minute Close & 375840 & 10 & 2 \\
FOREX eursek day High & 1837 & 10 & 2 \\
FOREX usdjpy minute Close & 375840 & 10 & 2 \\
FOREX eurhkd day High & 1832 & 10 & 2 \\
FOREX eurpln hour Close & 43825 & 10 & 2 \\
FOREX eurcad minute Close & 375840 & 10 & 2 \\
FOREX eurhuf hour Close & 43825 & 10 & 2 \\
FOREX audusd day Close & 1834 & 10 & 2 \\
FOREX chfsgd minute High & 375840 & 10 & 2 \\
FOREX eurrub day High & 1832 & 10 & 2 \\
FOREX chfjpy minute High & 375840 & 10 & 2 \\
FOREX cadchf day High & 1831 & 10 & 2 \\
FOREX audnzd minute Close & 375840 & 10 & 2 \\
FOREX usddkk minute Close & 375840 & 10 & 2 \\
FOREX gbpusd minute High & 375840 & 10 & 2 \\
FOREX eurhuf day Close & 1834 & 10 & 2 \\
FOREX eurnok minute Close & 375840 & 10 & 2 \\
FOREX usdcad day High & 1833 & 10 & 2 \\
FOREX eurjpy day Close & 1832 & 10 & 2 \\
FOREX cadchf minute Close & 375840 & 10 & 2 \\
FOREX audsgd day High & 1832 & 10 & 2 \\
FOREX usdchf minute Close & 375840 & 10 & 2 \\
FOREX eurjpy minute Close & 375840 & 10 & 2 \\
FOREX eursgd hour Close & 43825 & 10 & 2 \\
FOREX eurtry hour High & 43825 & 10 & 2 \\
FOREX eurhuf day High & 1834 & 10 & 2 \\
FOREX eursek minute Close & 375840 & 10 & 2 \\
FOREX audsgd hour Close & 43825 & 10 & 2 \\
FOREX audcad hour High & 43825 & 10 & 2 \\
FOREX gbpusd day High & 1834 & 10 & 2 \\
FOREX eurtry day Close & 1832 & 10 & 2 \\
FOREX eurgbp day High & 1835 & 10 & 2 \\
FOREX cadjpy hour Close & 43825 & 10 & 2 \\
FOREX audcad day Close & 1834 & 10 & 2 \\
FOREX audjpy minute High & 375840 & 10 & 2 \\
FOREX eurtry minute Close & 375840 & 10 & 2 \\
FOREX eurnok hour High & 43825 & 10 & 2 \\
FOREX audchf minute High & 375840 & 10 & 2 \\
FOREX eurtry hour Close & 43825 & 10 & 2 \\
FOREX eurhuf minute High & 375840 & 10 & 2 \\
FOREX usdcad minute Close & 375840 & 10 & 2 \\
FOREX eurhkd minute Close & 375840 & 10 & 2 \\
FOREX eurjpy hour High & 43825 & 10 & 2 \\
FOREX eurdkk minute High & 375840 & 10 & 2 \\
FOREX eursek hour High & 43825 & 10 & 2 \\
FOREX usdchf hour High & 43825 & 10 & 2 \\
FOREX audcad hour Close & 43825 & 10 & 2 \\
FOREX usdjpy hour Close & 43825 & 10 & 2 \\
FOREX eurdkk day Close & 1836 & 10 & 2 \\
FOREX gbpusd day Close & 1834 & 10 & 2 \\
FOREX eurtry day High & 1832 & 10 & 2 \\
FOREX eurgbp minute Close & 375840 & 10 & 2 \\
FOREX eurpln hour High & 43825 & 10 & 2 \\
FOREX audnzd day High & 1832 & 10 & 2 \\
FOREX eurnzd minute High & 375840 & 10 & 2 \\
FOREX cadjpy day Close & 1834 & 10 & 2 \\
FOREX eurusd day Close & 1837 & 10 & 2 \\
FOREX eurjpy minute High & 375840 & 10 & 2 \\
FOREX usdchf hour Close & 43825 & 10 & 2 \\
FOREX nzdusd minute Close & 375840 & 10 & 2 \\
FOREX gbpusd minute Close & 375840 & 10 & 2 \\
FOREX eurrub minute Close & 375840 & 10 & 2 \\
FOREX usdjpy day High & 1835 & 10 & 2 \\
FOREX usdcad minute High & 375840 & 10 & 2 \\
FOREX eurhkd hour Close & 43825 & 10 & 2 \\
FOREX cadjpy minute Close & 375840 & 10 & 2 \\
FOREX eursgd day High & 1832 & 10 & 2 \\
FOREX audcad minute High & 375840 & 10 & 2 \\
FOREX eurchf day High & 1833 & 10 & 2 \\
FOREX gbpusd hour Close & 43825 & 10 & 2 \\
FOREX eurrub hour High & 43825 & 10 & 2 \\
FOREX nzdusd minute High & 375840 & 10 & 2 \\
FOREX audjpy hour Close & 43825 & 10 & 2 \\
FOREX eurgbp minute High & 375840 & 10 & 2 \\
FOREX audusd minute High & 375840 & 10 & 2 \\
FOREX audchf minute Close & 375840 & 10 & 2 \\
FOREX eurnok day Close & 1837 & 10 & 2 \\
FOREX audsgd minute Close & 375840 & 10 & 2 \\
FOREX cadchf day Close & 1831 & 10 & 2 \\
FOREX euraud minute Close & 375840 & 10 & 2 \\
FOREX eurrub day Close & 1832 & 10 & 2 \\
FOREX usddkk hour High & 43825 & 10 & 2 \\
FOREX audusd minute Close & 375840 & 10 & 2 \\
FOREX euraud day Close & 1834 & 10 & 2 \\
FOREX eurrub minute High & 375840 & 10 & 2 \\
FOREX chfsgd hour High & 43825 & 10 & 2 \\
FOREX eurpln day Close & 1832 & 10 & 2 \\
FOREX audnzd minute High & 375840 & 10 & 2 \\
FOREX eurcad minute High & 375840 & 10 & 2 \\
FOREX eurgbp hour Close & 43825 & 10 & 2 \\
FOREX audnzd hour High & 43825 & 10 & 2 \\
FOREX eurnzd day Close & 1832 & 10 & 2 \\
FOREX usdcad hour High & 43825 & 10 & 2 \\
FOREX nzdusd day Close & 1828 & 10 & 2 \\
FOREX euraud hour Close & 43825 & 10 & 2 \\
FOREX nzdusd hour Close & 43825 & 10 & 2 \\
FOREX cadjpy hour High & 43825 & 10 & 2 \\
FOREX euraud hour High & 43825 & 10 & 2 \\
FOREX nzdusd day High & 1828 & 10 & 2 \\
FOREX usdcad day Close & 1833 & 10 & 2 \\
FOREX eurdkk hour Close & 43825 & 10 & 2 \\
FOREX cadchf minute High & 375840 & 10 & 2 \\
FOREX audjpy minute Close & 375840 & 10 & 2 \\
FOREX cadjpy day High & 1834 & 10 & 2 \\
FOREX cadchf hour Close & 43825 & 10 & 2 \\
FOREX eurnok minute High & 375840 & 10 & 2 \\
FOREX chfsgd day Close & 1832 & 10 & 2 \\
FOREX eurchf hour High & 43825 & 10 & 2 \\
FOREX audusd hour High & 43825 & 10 & 2 \\
FOREX eurusd minute High & 375840 & 10 & 2 \\
FOREX eursek day Close & 1837 & 10 & 2 \\
FOREX eurdkk day High & 1836 & 10 & 2 \\
FOREX audsgd day Close & 1832 & 10 & 2 \\
FOREX eursek minute High & 375840 & 10 & 2 \\
FOREX usdjpy hour High & 43825 & 10 & 2 \\
FOREX eurgbp day Close & 1835 & 10 & 2 \\
FOREX chfjpy day High & 1832 & 10 & 2 \\
FOREX eurchf minute High & 375840 & 10 & 2 \\
FOREX eurnzd minute Close & 375840 & 10 & 2 \\
FOREX audcad minute Close & 375840 & 10 & 2 \\
FOREX eurtry minute High & 375840 & 10 & 2 \\
FOREX eurdkk hour High & 43825 & 10 & 2 \\
FOREX audjpy day Close & 1832 & 10 & 2 \\
FOREX usdchf day Close & 1835 & 10 & 2 \\
FOREX eurnok hour Close & 43825 & 10 & 2 \\
FOREX eurusd hour Close & 43825 & 10 & 2 \\
FOREX eurrub hour Close & 43825 & 10 & 2 \\
FOREX eurnok day High & 1837 & 10 & 2 \\
FOREX chfsgd day High & 1832 & 10 & 2 \\
FOREX audsgd hour High & 43825 & 10 & 2 \\
FOREX euraud day High & 1834 & 10 & 2 \\
FOREX audnzd day Close & 1832 & 10 & 2 \\
FOREX eurpln day High & 1832 & 10 & 2 \\
FOREX eursgd minute Close & 375840 & 10 & 2 \\
FOREX chfjpy hour Close & 43825 & 10 & 2 \\
FOREX usddkk hour Close & 43825 & 10 & 2 \\
FOREX eurhkd day Close & 1832 & 10 & 2 \\
FOREX eurusd hour High & 43825 & 10 & 2 \\
FOREX eursgd day Close & 1832 & 10 & 2 \\
FOREX audchf day High & 1833 & 10 & 2 \\
FOREX eurdkk minute Close & 375840 & 10 & 2 \\
FOREX eurchf hour Close & 43825 & 10 & 2 \\
FOREX audusd hour Close & 43825 & 10 & 2 \\
FOREX gbpusd hour High & 43825 & 10 & 2 \\
FOREX chfsgd minute Close & 375840 & 10 & 2 \\
FOREX chfjpy hour High & 43825 & 10 & 2 \\
FOREX audjpy day High & 1832 & 10 & 2 \\
FOREX eurnzd hour High & 43825 & 10 & 2 \\
FOREX nzdusd hour High & 43825 & 10 & 2 \\
FOREX chfsgd hour Close & 43825 & 10 & 2 \\
FOREX eurnzd hour Close & 43825 & 10 & 2 \\
FOREX audsgd minute High & 375840 & 10 & 2 \\
FOREX audchf hour Close & 43825 & 10 & 2 \\
FOREX eurjpy hour Close & 43825 & 10 & 2 \\
FOREX usddkk minute High & 375840 & 10 & 2 \\
FOREX eurcad hour Close & 43825 & 10 & 2 \\
FOREX usdchf minute High & 375840 & 10 & 2 \\
FOREX eursgd hour High & 43825 & 10 & 2 \\
FOREX eurchf day Close & 1833 & 10 & 2 \\
FOREX eurhuf minute Close & 375840 & 10 & 2 \\
FOREX eursek hour Close & 43825 & 10 & 2 \\
FOREX audnzd hour Close & 43825 & 10 & 2 \\
FOREX usddkk day Close & 1832 & 10 & 2 \\
Indian pines & 9144 & 220 & 8 \\
telco customer churn & 7043 & 3 & 2 \\
compas two years & 5278 & 7 & 2 \\
SantanderCustomerSatisfaction & 200000 & 200 & 2 \\
sf police incidents & 538638 & 1 & 2 \\
hls4ml lhc jets hlf & 830000 & 16 & 5 \\
Higgs & 1000000 & 28 & 2 \\
1StudentPerfromance & 1000 & 3 & 2 \\
Census Augmented  & 1000000 & 6 & 2 \\
students scores & 1000 & 3 & 2 \\
ibm employee attrition & 1470 & 26 & 2 \\
ibm employee performance & 1470 & 25 & 2 \\
eucalyptus & 4331 & 5 & 4 \\
KDDCup09 upselling & 5032 & 34 & 2 \\
rl & 4970 & 5 & 2 \\
kdd ipums la 97 small & 5188 & 15 & 2 \\
MagicTelescope & 13376 & 10 & 2 \\
california & 20634 & 8 & 2 \\
wine & 2554 & 11 & 2 \\
road safety & 111762 & 29 & 2 \\
spambase reproduced & 4601 & 57 & 2 \\
compass & 16644 & 8 & 2 \\
UCI churn & 3333 & 16 & 2 \\
Bank marketing data set UCI & 45211 & 7 & 2 \\
california seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 8 & 2 \\
california seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 8 & 2 \\
california seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 8 & 2 \\
california seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 8 & 2 \\
california seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 8 & 2 \\
wine seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 11 & 2 \\
wine seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 11 & 2 \\
wine seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 11 & 2 \\
wine seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 11 & 2 \\
electricity seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 7 & 2 \\
electricity seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 7 & 2 \\
electricity seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 7 & 2 \\
electricity seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 7 & 2 \\
wine seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 11 & 2 \\
covertype seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 10 & 2 \\
covertype seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 10 & 2 \\
electricity seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 7 & 2 \\
covertype seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 10 & 2 \\
pol seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 26 & 2 \\
covertype seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 10 & 2 \\
covertype seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 10 & 2 \\
pol seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 26 & 2 \\
pol seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 26 & 2 \\
pol seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 26 & 2 \\
pol seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 26 & 2 \\
house 16H seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 16 & 2 \\
house 16H seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 16 & 2 \\
house 16H seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 16 & 2 \\
house 16H seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 16 & 2 \\
house 16H seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 16 & 2 \\
kdd ipums la 97 small seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 20 & 2 \\
kdd ipums la 97 small seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 20 & 2 \\
kdd ipums la 97 small seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 20 & 2 \\
kdd ipums la 97 small seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 20 & 2 \\
kdd ipums la 97 small seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 20 & 2 \\
MagicTelescope seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 10 & 2 \\
MagicTelescope seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 10 & 2 \\
MagicTelescope seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 10 & 2 \\
MagicTelescope seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 10 & 2 \\
bank marketing seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 7 & 2 \\
bank marketing seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 7 & 2 \\
bank marketing seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 7 & 2 \\
bank marketing seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 7 & 2 \\
phoneme seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 5 & 2 \\
MagicTelescope seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 10 & 2 \\
phoneme seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 5 & 2 \\
phoneme seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 5 & 2 \\
phoneme seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 5 & 2 \\
phoneme seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 5 & 2 \\
MiniBooNE seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 50 & 2 \\
MiniBooNE seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 50 & 2 \\
MiniBooNE seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 50 & 2 \\
MiniBooNE seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 50 & 2 \\
MiniBooNE seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 50 & 2 \\
Higgs seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 24 & 2 \\
Higgs seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 24 & 2 \\
Higgs seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 24 & 2 \\
Higgs seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 24 & 2 \\
eye movements seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 20 & 2 \\
eye movements seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 20 & 2 \\
eye movements seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 20 & 2 \\
eye movements seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 20 & 2 \\
eye movements seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 20 & 2 \\
jannis seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 54 & 2 \\
jannis seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 54 & 2 \\
jannis seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 54 & 2 \\
jannis seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 54 & 2 \\
jannis seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 54 & 2 \\
rl seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 5 & 2 \\
rl seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 5 & 2 \\
rl seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 5 & 2 \\
rl seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 5 & 2 \\
rl seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 5 & 2 \\
road safety seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 29 & 2 \\
road safety seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 29 & 2 \\
road safety seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 29 & 2 \\
road safety seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 29 & 2 \\
compass seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 8 & 2 \\
road safety seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 29 & 2 \\
compass seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 8 & 2 \\
compass seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 8 & 2 \\
KDDCup09 upselling seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 34 & 2 \\
compass seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 8 & 2 \\
compass seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 8 & 2 \\
KDDCup09 upselling seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 34 & 2 \\
KDDCup09 upselling seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 34 & 2 \\
KDDCup09 upselling seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 34 & 2 \\
yeast seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 1484 & 8 & 10 \\
yeast seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 1484 & 8 & 10 \\
yeast seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 1484 & 8 & 10 \\
yeast seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 1484 & 8 & 10 \\
KDDCup09 upselling seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 34 & 2 \\
yeast seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 1484 & 8 & 10 \\
wilt seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 5 & 2 \\
wilt seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 5 & 2 \\
wilt seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 5 & 2 \\
numerai28 6 seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 21 & 2 \\
numerai28 6 seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 21 & 2 \\
numerai28 6 seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 21 & 2 \\
numerai28 6 seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 21 & 2 \\
numerai28 6 seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 21 & 2 \\
steel plates fault seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 1941 & 27 & 7 \\
steel plates fault seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 1941 & 27 & 7 \\
steel plates fault seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 1941 & 27 & 7 \\
steel plates fault seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 1941 & 27 & 7 \\
steel plates fault seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 1941 & 27 & 7 \\
dilbert seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 5 \\
dilbert seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 5 \\
dilbert seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 5 \\
dilbert seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 5 \\
dilbert seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 5 \\
fabert seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 7 \\
fabert seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 7 \\
fabert seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 7 \\
fabert seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 7 \\
jasmine seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 6 & 2 \\
jasmine seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 6 & 2 \\
jasmine seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 6 & 2 \\
jasmine seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 6 & 2 \\
airlines seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 3 & 2 \\
fabert seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 7 \\
airlines seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 3 & 2 \\
jasmine seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 6 & 2 \\
airlines seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 3 & 2 \\
airlines seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 3 & 2 \\
airlines seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 3 & 2 \\
gina seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
gina seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
gina seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
gina seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
gina seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
ozone level 8hr seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 72 & 2 \\
ozone level 8hr seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 72 & 2 \\
ozone level 8hr seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 72 & 2 \\
ozone level 8hr seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 72 & 2 \\
ozone level 8hr seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 72 & 2 \\
madeline seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
madeline seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
madeline seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
madeline seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
madeline seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
philippine seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
philippine seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
philippine seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
philippine seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
philippine seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
qsar biodeg seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 1055 & 41 & 2 \\
qsar biodeg seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 1055 & 41 & 2 \\
qsar biodeg seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 1055 & 41 & 2 \\
qsar biodeg seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 1055 & 41 & 2 \\
qsar biodeg seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 1055 & 41 & 2 \\
pc4 seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 1458 & 37 & 2 \\
pc4 seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 1458 & 37 & 2 \\
pc4 seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 1458 & 37 & 2 \\
pc4 seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 1458 & 37 & 2 \\
pc4 seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 1458 & 37 & 2 \\
kc1 seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 21 & 2 \\
kc1 seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 21 & 2 \\
kc1 seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 21 & 2 \\
kc1 seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 21 & 2 \\
segment seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 16 & 7 \\
segment seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 16 & 7 \\
segment seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 16 & 7 \\
segment seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 16 & 7 \\
segment seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 16 & 7 \\
Bioresponse seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
kc1 seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 21 & 2 \\
Bioresponse seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
Bioresponse seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
Bioresponse seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
Bioresponse seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
churn seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 16 & 2 \\
churn seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 16 & 2 \\
churn seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 16 & 2 \\
churn seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 16 & 2 \\
first order theorem proving seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 51 & 6 \\
churn seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 16 & 2 \\
first order theorem proving seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 51 & 6 \\
first order theorem proving seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 51 & 6 \\
first order theorem proving seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 51 & 6 \\
first order theorem proving seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 51 & 6 \\
sylvine seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 20 & 2 \\
sylvine seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 20 & 2 \\
sylvine seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 20 & 2 \\
sylvine seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 20 & 2 \\
sylvine seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 20 & 2 \\
christine seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 96 & 2 \\
christine seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 96 & 2 \\
christine seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 97 & 2 \\
christine seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
christine seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 99 & 2 \\
wine quality white seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 11 & 7 \\
wine quality white seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 11 & 7 \\
wine quality white seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 11 & 7 \\
wine quality white seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 11 & 7 \\
wine quality white seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 11 & 7 \\
Fashion MNIST seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 10 \\
Fashion MNIST seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 10 \\
Fashion MNIST seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 10 \\
Fashion MNIST seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 10 \\
Fashion MNIST seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 10 \\
nomao seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 75 & 2 \\
nomao seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 77 & 2 \\
nomao seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 75 & 2 \\
nomao seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 74 & 2 \\
jungle chess 2pcs raw endgame complete seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 6 & 3 \\
jungle chess 2pcs raw endgame complete seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 6 & 3 \\
volkert seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 10 \\
volkert seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 10 \\
volkert seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 10 \\
volkert seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 10 \\
jungle chess 2pcs raw endgame complete seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 6 & 3 \\
volkert seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 10 \\
robert seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 10 \\
robert seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 10 \\
robert seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 10 \\
robert seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 10 \\
robert seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 10 \\
shuttle seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 9 & 5 \\
shuttle seed 1 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 9 & 5 \\
shuttle seed 2 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 9 & 5 \\
shuttle seed 3 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 9 & 5 \\
shuttle seed 4 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 9 & 5 \\
guillermo seed 0 nrows 2000 nclasses 10 ncols 100 stratify True & 2000 & 100 & 2 \\
\bottomrule
\end{supertabular}


==> tex/tables/xor_table.tex <==
\begin{table}
  \begin{center}
    \caption{Relative error of \method~(trained on XOR Level 1 with 15\% noise) on XOR datasets with level=$\{1,2\}$ and label flipping noise rate=$\{0\%, 5\%, 10\%, 15\%, 20\%, 25\%\}$. 
    % Error gap calculated as ($100\% - \text{label noise rate} - \text{fitting accuracy}$).
    }
    %\vspace{-3mm}
    \small
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{l|cccccc} 
      \toprule
      Noise & 0\% & 5\% & 10\% & 15\% & 20\% & 25\% \\
      \midrule
      XOR L1 & 4.54  & 4.14 & 3.84 & 3.50 & 3.08 & 2.61\\
      XOR L2 & 12.29 & 10.91 & 9.33 & 7.54 & 5.21 & 2.41\\
      %XOR L1 & 95.46  & 90.86 & 86.16 & 81.50 & 76.92 & 72.39\\
      %XOR L2 & 87.71 & 84.09 & 80.67 & 77.46 & 74.79 & 72.59\\
      
      \bottomrule
    \end{tabular}
    % }
    \label{tab:xor_table}
  \end{center}
  %\vspace{-3mm}
\end{table}
